Active Learning for Video Description With Cluster-Regularized Ensemble Ranking

Automatic video captioning aims to train models to generate text descriptions for all segments in a video, however, the most effective approaches require large amounts of manual annotation which is slow and expensive. Active learning is a promising way to efficiently build a training set for video captioning tasks while reducing the need to manually label uninformative examples. In this work we both explore various active learning approaches for automatic video captioning and show that a cluster-regularized ensemble strategy provides the best active learning approach to efficiently gather training sets for video captioning. We evaluate our approaches on the MSR-VTT and LSMDC datasets using both transformer and LSTM based captioning models and show that our novel strategy can achieve high performance while using up to 60% fewer training data than the strong state of the art baselines.

==> tex_figures/qual_fig.tex <==
% \begin{figure}
    
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=0.5\textwidth]{figs/ex_1.png} \\
%          {\fontfamily{qcr}\selectfont\tiny a clip of the video game minecraft}
%          \includegraphics[width=0.5\textwidth]{figs/ex_2.png} \\
%          {\fontfamily{qcr}\selectfont\tiny a person is playing a computer online game}
%          \caption{Validation}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/ex_8.png}
%          {\fontfamily{qcr}\selectfont\tiny a short 3d rendering taken in either a video game or movie}
%          \caption{Agreement}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/ex_4.png}
%          {\fontfamily{qcr}\selectfont\tiny a man provides a voiceover description of his actions while playing a video game}
%          \caption{Clustered Agreement}
%      \end{subfigure}
%      \newline
%      \newline
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/ex_3.png}
%          {\fontfamily{qcr}\selectfont\tiny an elderly man playing a fighting video game with his wife}
%          \caption{Entropy}
%      \end{subfigure}
%      \qquad
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=0.5\textwidth]{figs/ex_6.png} \\
%          {\fontfamily{qcr}\selectfont\tiny a cartoon of puppies and a train}
%          \includegraphics[width=0.5\textwidth]{figs/ex_7.png} \\
%          {\fontfamily{qcr}\selectfont\tiny amazing sports plays caught on camera}
%          \caption{Random}
%      \end{subfigure}
%     \caption{Above, we visualize some of the selected samples in the first iteration by the active learning and random methods in a particular cluster (Cluster 237). We can clearly see that the active learning methods are selecting more relevant samples to the validation set in the particular cluster (all of the samples in the cluster in the validation set pertain to video gaming), over the random method which is ignoring irrelevant samples in the cluster. \textcolor{red}{TODO: Update This Figure}}
%     \label{fig:cluster_vis}
% \end{figure}

